Language Model Cascades: Token-level uncertainty and beyond

Recent advances in language models (LMs) have led to significant improvements in quality on complex NLP tasks, but at the expense of increased inference costs. Cascading offers a simple strategy to achieve more favorable cost-quality tradeoffs: here, a small model is invoked for most "easy" instances, while a few "hard" instances are deferred to the large model. While the principles underpinning cascading are well-studied for classification tasks - with deferral based on predicted class uncertainty favored theoretically and practically - a similar understanding is lacking for generative LM tasks. In this work, we initiate a systematic study of deferral rules for LM cascades. We begin by examining the natural extension of predicted class uncertainty to generative LM tasks, namely, the predicted sequence uncertainty. We show that this measure suffers from the length bias problem, either over- or under-emphasizing outputs based on their lengths. This is because LMs produce a sequence of uncertainty values, one for each output token; and moreover, the number of output tokens is variable across examples. To mitigate this issue, we propose to exploit the richer token-level uncertainty information implicit in generative LMs. We argue that naive predicted sequence uncertainty corresponds to a simple aggregation of these uncertainties. By contrast, we show that incorporating token-level uncertainty through learned post-hoc deferral rules can significantly outperform such simple aggregation strategies, via experiments on a range of natural language benchmarks with FLAN-T5 models. We further show that incorporating embeddings from the smaller model and intermediate layers of the larger model can give an additional boost in the overall cost-quality tradeoff.

==> conclusion.tex <==
%
\label{sec:background-uq-lm}

%


%



==> confidence_measures_old.tex <==
%
\subsection{Cascading language models: formalism}

Cascades of generative LMs largely follow the setup in~\S\ref{sec:background-cascades}, except that we now consider \emph{probabilistic} models over \emph{sequences}.
% Further, the measure of \emph{quality} of a candidate response is generally challenging.
Concretely, suppose we have $K$ language models $p^{(1)}, \ldots, p^{(K)}$,
with inference costs (e.g., latencies) $c^{(1)}, \ldots, c^{(K)}$.
Similarly,
suppose $q \colon \mathscr{V}^m \times \Delta( \mathscr{V}^n ) \to \Real_+$ is a measure of the \emph{quality} of a given distribution over responses for a given prompt.
A cascade 
$p^{\rm cas}$ of these models
is parameterised by
deferral rules $r^{(1)}, \ldots, r^{(K - 1)} \colon \mathscr{V} \to \{ 0, 1 \}$,
% where $r^{(k)}( \boldsymbol{x} ) \geq r^{(k + 1)}( \boldsymbol{x} )$,
and is given by:
$$ p^{\rm cas}( \cdot \mid \boldsymbol{x} ) = 
\sum_{k \in [K]} \1( s( \boldsymbol{x} ) = k ) \cdot p^{(k)}( \cdot \mid \boldsymbol{x} ). $$
% where the \emph{selection} function $s( \boldsymbol{x} ) \defEq \sum_{k \in [K]} \prod_{k' = 1}^{k - 1} \1( r^{(k')}( \boldsymbol{x} ) = 1 ) \cdot \1( r^{(k)}( \boldsymbol{x} ) = 0 )$, with $r^{(K)}( \boldsymbol{x} ) = 1$ by convention.
Given an input sequence $\boldsymbol{x}$,
an LM cascade results in quality and cost
\begin{align*}
    Q( \boldsymbol{x}, p^{\rm cas}( \cdot \mid \boldsymbol{x} ) ) &\defEq \sum_{k \in [K]} \1( s( \boldsymbol{x} ) = k ) \cdot q( \boldsymbol{x}, p^{(k)}( \cdot \mid \boldsymbol{x} ) ) \\
    C( \boldsymbol{x}, p^{\rm cas}( \cdot \mid \boldsymbol{x} ) ) &\defEq \sum_{k \in [K]} \1( s( \boldsymbol{x} ) \geq k ) \cdot c^{(k)}. 
\end{align*}
% Ideally, one seeks to maximise {quality} 
% given a budget $B$ on total {inference cost}:
% $$ \min_{r^{(1)}, \ldots, r^{(K - 1)}} \mathbb{E}_{\boldsymbol{x}}[ Q( \boldsymbol{x}, p^{\rm cas}( \cdot \mid \boldsymbol{x} ) ) ] \colon \mathbb{E}_{\boldsymbol{x}}[ C( \boldsymbol{x}, p^{\rm cas}( \cdot \mid \boldsymbol{x} ) ) ] \leq B. $$
% To achieve this, a key question is how to design suitable deferral rules.


%
\subsection{Confidence measures for language models}

To design a suitable deferral rule for LM cascading,
a natural starting point is to mimic the maximum predictive probability~\eqref{eqn:max-softmax}:
we may compute
\begin{equation}
    \label{eqn:max-softmax-seq}
    \gamma^{(k)}( \boldsymbol{x} ) \defEq \max_{\boldsymbol{y'}} p^{( k )}( \boldsymbol{y}' \mid \boldsymbol{x} ),
\end{equation}
i.e., the probability of the most likely sequence.
Compared to the classification setting, this requires searching over the space of all possible sequences;
however, efficient approximations via greedy or beam search are feasible.

Given that this deferral rule tracks closely with the well-established~\eqref{eqn:max-softmax}, 
it is tempting to conclude that this emphatically solves the LM cascade problem.
However, we make two subtle observations that suggest a closer investigation is warranted.

First, LMs are known to suffer from the \emph{length bias} problem~\citep{Murray:2018,Adiwardana:2020}:
shorter, lower quality responses may receive a higher probability than longer, higher quality responses.
This may be seen as a consequence of the fact that each 
$p( \cdot \mid \boldsymbol{x}, y_{1}, \ldots, y_{i} )$ provides an \emph{imperfect} estimate of a notional ``true'' probability $p^{*}( \cdot \mid \boldsymbol{x}, y_{1}, \ldots, y_{i} )$ over responses,
and that errors in these estimates accumulate as sequences grow.
A common heuristic to resolve this is to compute the \emph{length normalised} log-probability $\frac{1}{| {\rm len}( \boldsymbol{y} ) |} \cdot \log p( \boldsymbol{y} \mid \boldsymbol{x} )$;
one may naturally wonder if such correction is similarly important for cascading.

Second, computing the probability of an entire sequence may mask settings where \emph{individual tokens} are highly uncertain,
even if the entire sequence has reasonably high probability.
Such token-level uncertainty may be highly important in certain settings such as fact-answering:
here, an LM may be (correctly) highly confident on articles and other grammatical primitives, but these are of less interest than confidence on tokens corresponding to entities (say).

%
\textbf{Token-based uncertainty}.
The above suggest there is minimally value in considering the following generalisation of the maximal sequence probability:
\todoakm{Better notation}
$$ \zeta( \boldsymbol{x} ) \defEq F( {\tt agg}( p( \cdot \mid \boldsymbol{x} ), p( \cdot \mid \boldsymbol{x}, y_1 ), \ldots, p( \cdot \mid \boldsymbol{x}, y_1, \ldots, y_{n - 1} ) ) ). $$
Here, {\tt agg} is some \emph{aggregation} function that operates on an arbitrary-length sequence of vectors, each of which provides a probability distribution over the vocabulary.
In the simplest case, this could be the row-wise mean, median, or other quantile.
The function $F( \cdot )$ further processes the resulting fixed length vector into a scalar measure of confidence.

%
\textbf{Embedding-based uncertainty}.
A natural generalisation of the above is to consider the intermediate \emph{token embeddings} produced by an LM.
Previous work~\citep{Ren:2023} has shown the value of
such embeddings for \emph{selective generation},
\todoakm{Mention selective generation in Background}
and the related problem of \emph{out-of-distribution} detection.
We note that for encoder-decoder models such as T5, 
such embeddings can be from either the encoder, decoder, or both.

%
\textbf{Consensus-based}.
One limitation of Equation~\ref{eqn:max-softmax-seq} 
is that it considers a \emph{single} output sequence, namely, the most likely one.
However, as there are many sequences that have similar meaning, it is intuitively more reliable to consider drawing \emph{multiple} sequences from $p( \cdot \mid \boldsymbol{x} )$.
One may then assess the \emph{consensus} in resulting predictions to measure confidence~\citep{Wang:2023,Xiao:2021,Chen:2023b};
this can help distinguish between models that are locally diffuse versus peaked around a candidate sequence.

%
\textbf{Deep ensembles and dropout}.
\citep{Landeghem:2022,Wang:2019,Gleave:2022}

%
\textbf{Semantic entropy}.
\citep{Kuhn:2023}

%
\textbf{Generative uncertainty}.
The above has largely focussed on generalising the standard maximum predictive probability~\eqref{eqn:max-softmax} from classification to the LM setting.
While this by itself leads to a rich array of possible confidence measures,
LMs intriguingly offer a wholly new possible means of assessing confidence:
one may directly probe the model to obtain its score on a string such as {\tt ``I don't know''}~\citep{Kadavath:2022}.
\todoakm{What exactly does that paper propose?}
It is not clear \emph{a-priori} how such \emph{generative} uncertainty measures fare against more classical softmax-based measures.

%
\textbf{Post-hoc calibration/Answer- and length-bias calibration}.
\citep{Zhao:2021,Holtzman:2021,Kumar:2022,Murray:2018,Mielke:2022,Jiang:2021}

%
\textbf{Other work}.
\citep{Zhao:2023} proposed sequence-level calibration.
\citep{Malinin:2021,Tan:2019,Jagannatha:2020}


==> experiments.tex <==
%%%
\subsection{Setup}

%
\textbf{Models}.
FLAN-T5~\citep{Chung:2022} models, which are T5 models~\citep{Raffel:2020} that have undergone instruction tuning~\citep{Wei:2022}.

%
\textbf{Datasets}.
We consider over 15 datasets corresponding to a range of different language tasks:
% \begin{enumerate}[label=(\arabic*),itemsep=0pt,topsep=0pt]
    % \item 
    \emph{Classification}
    (IMDb~\citep{Maas:2011},
    SuperGLUE~\citep{Wang:2019b},
    MNLI~\citep{Williams:2018},
    ANLI~\citep{Nie:2020},
    HellaSwag~\citep{Zellers:2019});
    \emph{Question answering} 
    (Physical IQa,
    TriviaQA~\citep{Joshi:2017},
    NaturalQA~\citep{Kwiatkowski:2019},
    TyDiQA \{ ID, SW, FI \}~\citep{Clark:2020});
    % \item 
    % \textbf{Summarisation}: 
    % \item 
    \emph{Reading comprehension}
    (Lambada~\citep{Paperno:2016},
    SQuAD~\citep{Rajpurkar:2016},
    StoryCloze~\citep{Mostafazadeh:2016});
    % \item 
    \emph{Translation}
    (WMT EN $\to$ FR, DE $\to$ FR, and FR $\to$ EN);
    \emph{Common-sense reasoning}
    (Winogrande~\citep{Sakaguchi:2020}).
% \end{enumerate}

% Ranking Tasks: 
% Piqa
% Storycloze
% Copa
% Imdb
% Boolq
% Winogrande
% Mnli
% Anli-r1
% Anli-r2
% Anli-r3
% Hellaswag

% Generation Tasks:
% Triviaqa
% Naturalqa
% Lambada
% Squad
% Tydiqa-id
% Tydiqa-sw
% Tydiqa-fi

% Language Translation Tasks: 
% Wmt-en-fr
% Wmt-de-fr
% Wmt-fr-en

%
\textbf{Baselines}.
We compare
\emph{random cascading},
regular \emph{confidence-based cascading},
and representative methods from each option discussed in \S\ref{sec:confidence_measures}:
\begin{enumerate}[label=(\arabic*)]
    \item \emph{Token-confidence based}: 
    \item \emph{Embedding-based}: 
\end{enumerate}

%
\textbf{Metrics}.
We primarily summarize performance using the \emph{area under the cost-quality curve}.


%%%
\subsection{Results}

\textbf{Does sequence-level confidence suffice?}

%
\textbf{Is router training useful?}


%
% \textbf{Cascades versus routers}.

% %
% \textbf{Training supervision}.

% %
% \textbf{Uncertainty type}.

% %
% \begin{table}[!t]
%     \centering
    
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{@{}llllll|llll|lll|l@{}}
%         \toprule
%         \textbf{Method} & \textbf{IMDb} & \textbf{SuperGLUE} & \textbf{MNLI} & \textbf{ANLI} & \textbf{HellaSwag} & \textbf{PIQA} & \textbf{TriviaQA} & \textbf{NaturalQA} & \textbf{TyDiQA} & \textbf{Lambada} & \textbf{SQuAD} & \textbf{StoryCloze} & \textbf{WMT} \\
%         \toprule
%         \toprule
%         Confidence & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? \\
%         \midrule
%         Token-confidence & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? \\
%         Embedding & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? \\
%         Sampling & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? \\
%         Generation & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? & ??.? \\
%         \bottomrule
%     \end{tabular}
%     }

%     \caption{Summary of area under cost-quality curve for different methods on all datasets.}
%     \label{tbl:results}
% \end{table}


==> intro_old.tex <==
Recent advances in generative language modelling have yielded a series of 
Transformer-based models 
with remarkably improved \emph{quality} on complex NLP tasks~\citep{Radford:2018,Raffel:2020,Brown:2020,Chowdhery:2022,Wei:2022,Chung:2022,Tay:2023,Anil:2023}.
Unfortunately, such models also involve significantly increased \emph{inference cost},
which has motivated a series of efforts at reducing the same~\citep{Pope:2022,Schuster:2022,Leviathan:2023,Chen:2023,Sheng:2023,Sun:2023}.

\emph{Cascading} is a simple strategy to achieve more favourable cost-quality tradeoffs
via \emph{adaptive} inference.
In a two-model cascade,
a small model is invoked for most ``easy'' instances, while 
a large model is invoked for a few ``hard'' instances.
To judge whether or not an input is ``easy'', 
a standard recipe is to employ the small model's prediction \emph{confidence},
as canonically measured by its softmax probability output.
Cascades
have been widely explored in the vision domain~\citep{Viola:2001,Trapeznikov:2013,Bolukbasi:2017,Huang:2018,Kag:2023,Jitkrittum:2023},
and
have seen increasing adoption within NLP~\citep{Mamou:2022,Varshney:2022,Khalili:2022,Dohan:2022,Chen:2023a}.

While the principles underpinning effective cascading are well-studied for \emph{classification},
a similar understanding is lacking for \emph{generative} LM tasks.
In particular, there is limited clarity on a central question: 
how does one best summarize model confidence across a \emph{variable} number of output tokens?
\todowj{Should we say that it is natural to take the sum (yielding the standard sequence probability) but it may not always be the best for cascading?}
In this paper, we aim to systematically study the issue of designing effective cascades for generative LMs.
To this end, we study the viability of a range of LM confidence measures to predict when to defer to a larger model.
Via experiments on a range of benchmarks with FLAN-T5 models, 
we find that incorporating \emph{token-level} uncertainty can significantly improve the cost-quality tradeoff of cascades
compared to na\"{i}ve example-level uncertainty, as typically employed in classification settings.
We further show that incorporating embeddings from the smaller model, and intermediate layer embeddings from the larger model can give additional performance boost.

\todoakm{Revisit this para}

In sum, our contributions are:
\todoakm{Revisit these}
\begin{enumerate}[label=(\roman*),itemsep=0pt,topsep=0pt,leftmargin=16pt]
    \item we provide a systematic overview of different approaches to measuring generative LM confidence,
    including input-, output-, and prompt-based strategies (\S\ref{sec:confidence_measures})
    
    \item based on the above, we propose a variety of distinct strategies to construct model cascades (\S\ref{sec:confidence_measures})
    
    \item we provide a systematic set of experiments on various NLP tasks, which demonstrate the value of incorporating token-level uncertainty (\S\ref{sec:router_experiments}).
\end{enumerate}

% For example, 
% how does one best summarize model confidence across a variable number of output tokens?
% % How do prompt-based confidence measures compare against raw softmax probabilities?
% Can one exploit the generative nature of LMs to obtain richer confidence estimates that simply studying the model's softmax probability estimates?
% \todoakm{We may not end up addressing this point}
% % Given that measuring the quality of LM generation is, at best, fraught with complexity, how can one assess the promise of a given cascading strategy?
% % \todoakm{Probably we are not going to offer anything new here}
% To the best of our knowledge, such questions have received limited prior study.
% \todoakm{A bit mixed: new analysis, or studying existing ideas?}
% While intuitive, a natural question is whether this simple confidence measure reliably captures LM confidence.


==> limitations.tex <==
One potential limitation of post-hoc deferral rule
training is that it may not work well if there is some distribution shift between the probability values in the train and test sets. It also may not work in settings where we have limited training data, especially where we use high dimensional features like embeddings.

==> old_abstract.tex <==
Recent advances in language model (LM) design has yielded a series of models
with remarkably improved \emph{quality} on complex NLP tasks,
but significantly increased \emph{inference cost}.
A simple strategy to achieve more favourable cost-quality tradeoffs is \emph{cascading}:
here, 
a small model is invoked for most ``easy'' instances, while 
a large model is invoked for a few ``hard'' instances.
% To judge whether or not an input is ``easy'', 
% a standard recipe is to employ the small model's \emph{confidence} in its prediction.
Typically, ``easy'' instances are those where the small model has high \emph{confidence} in its prediction.
% as measured by its softmax probability output.
% While intuitive, a natural question is whether this simple confidence measure reliably captures LM confidence.
% While cascades have been widely studied for classification,
While the principles underpinning effective cascading are well-studied for classification problems,
a similar understanding is lacking for generative tasks.
% there is limited understanding of how best to design them for generative tasks.
For example, 
how does one best summarise model confidence across a variable number of output tokens,
% and how do prompt-based confidence measures compare against measures derived from raw softmax probabilities?
and how can one exploit the generative nature of LMs to obtain richer confidence estimates?
In this paper, we study the viability of a range of alternate LM confidence measures for cascading.
Via experiments on a range of benchmarks with FLAN-T5 models, we find that incorporating \emph{token-level} uncertainty can significantly improve the cost-quality tradeoff of cascades.

% Uncertainty estimation is a long studied problem, and many metrics have been proposed to quantify uncertainty of a model for an input.
% Similarly, example hardness for a model has been quantified through different metrics.
% In another line of work, cascades are important for efficient inference. 
% Cascading also requires some form of uncertainty metric for the model and the example to decide whether to defer or not
% We conduct a systematic study of the effects of using different uncertainty metrics for cascades in deciding whether to defer or not across a wide variety of tasks in the language domain.
% We also propose a few metrics and evaluate their effectiveness for cascades.
% We find out that ... metrics are beneficial for effective cascades


==> related_work.tex <==
%\textbf{Efficient LM inference strategies.}
%
%While modern LMs yield remarkably high-quality predictions on a range of tasks,
%this comes at the price of a non-trivial increase in inference cost (e.g., latency).
%In response, there have been a number of proposals to mitigate this cost~\citep{Tay:2022,Menghani:2022}.

% Fortunately, several of these approaches can be applied in unison.
%Our interest is in \emph{model cascades}, a simple strategy that we describe next. 

==> table.tex <==

%
\begin{table}[!t]
    \centering
    
    \resizebox{\linewidth}{!}{
\begin{tabular}{@{}lS[table-format=0.3]S[table-format=0.3]S[table-format=0.3]S[table-format=0.3]S[table-format=0.3]S[table-format=0.3]S[table-format=0.3]@{}}
\toprule
\toprule
   {\bf Dataset} & {\bf\tt Random} &     {\bf\tt Chow-Sum} & {\bf\tt Chow-Average} & {\bf\tt Chow-Quantile-0} & {\bf\tt Chow-Quantile-0.4} & {\bf\tt Chow-Quantile-0.8} &       {\bf\tt Router} \\
\midrule
   ANLI-R1 &  0.501 &        0.524  &        0.519 &    \bfseries{0.534} &             0.515 &             0.515 & \bfseries{0.534} \\
   ANLI-R2 &  0.443 &        0.446 &        0.446 &    \bfseries{0.449} &             0.440 &             0.441 &        0.442 \\
   ANLI-R3 &  0.399 &        0.413 &        0.422 &           0.417 &      \bfseries{0.425} &             0.424 & \bfseries{0.425} \\
     BoolQ &  0.817 &        0.838 &        0.838 &           0.838 &             0.838 &             0.838 &        \bfseries{0.840} \\
      IMDb &  0.953 & \bfseries{0.964} & \bfseries{0.964} &    \bfseries{0.964} &      \bfseries{0.964} & \bfseries{0.964} & \bfseries{0.964} \\
   Lambada &  0.680 & \bfseries{0.703} &        0.702 &    \bfseries{0.703} &             0.694 &             0.687 &        0.701 \\
      MNLI &  0.644 &        0.627 &        0.642 &           0.631 &             0.677 &             0.691 & \bfseries{0.711} \\
%  naturalqa &  0.052 &        0.049 &        0.049 &           0.048 &             0.050 &             0.051 & \bfseries{0.056} \\
      PIQA &  0.705 &        0.712 &        0.708 &           0.715 &             0.706 &             0.705 & \bfseries{0.717} \\
     SQuaD &  0.401 &        0.410 &        0.408 &           \bfseries{0.410} &             0.399 &             0.398 &        0.409 \\
  TriviaQA &  0.084 &        0.073 &        0.087 &           0.073 &             0.088 &             0.086 & \bfseries{0.097} \\
 TydiQA-FI &  0.322 & \bfseries{0.332} &        0.322 &           0.328 &             0.318 &             0.312 &        0.331 \\
 TydiQA-ID &  0.230 & \bfseries{0.247} &        0.239 &           0.245 &             0.230 &             0.230 &        0.235 \\
 TyDiQA-SW &  0.155 &        \bfseries{0.170} &        0.147 &           0.166 &             0.141 &             0.140 &        0.163 \\
Winogrande &  0.633 &        0.648 &        0.648 &           0.648 &      \bfseries{0.649} &             0.648 &        0.648 \\
 WMT DE $\rightarrow$ FR &  0.390 &        0.390 &        0.392 &           0.391 &             0.396 &             0.401 & \bfseries{0.404} \\
 WMT EN $\rightarrow$ FR &  0.431 &        0.436 &        0.435 &           0.436 &             0.435 &             0.439 & \bfseries{0.441} \\
 WMT FR $\rightarrow$ EN &  0.601 &        0.618 &        0.595 &           0.618 &             0.595 &             0.614 & \bfseries{0.619} \\
\bottomrule
\end{tabular}
}
    \caption{Summary of area under the deferral curve for various methods.
    The post-hoc router approach is the most consistently performant method.}
    \label{tbl:area_under_curve}
\end{table}
